The landscape of QCD axion models

We review the landscape of QCD axion models. Theoretical constructions that extend the window for the axion mass and couplings beyond conventional regions are highlighted and classified. Bounds from cosmology, astrophysics and experimental searches are reexamined and updated.

==> 8.2_Outlook.tex <==

\begin{itemize} 
\item \emph{Topological defects.}
\LDL{Assessing the contribution to axion DM from topological defects (strings and domain walls)
remains a major unsettled question, which requires extensive numerical simulations 
of the string network evolution and its extrapolation from the PQ scale 
down to the QCD phase transition.  
To obtain the final axion DM relic abundance one 
has to include (on top of the standard VRM contribution) also  
the dynamics of domain walls formation when the axion mass is turned on,  
with the subsequent non-thermal axion production arising from the destruction of the 
string-wall network. Although this appears to be a remarkably difficult task, 
the importance of ending up with a reliable estimate cannot be overstated, 
since it would lead to a ``standard model of axion physics'' 
(based on a post-inflationary PQ breaking scenario with $N_{\rm DW} = 1$)
which would represent a crucial target for the scanning strategy of axion DM experiments.}
%\item Astro: Refined computation of the axion emissivity from SN, also in view 
%of  exploiting at best observations from the next  galactic SN explosion.  
%\bigskip 

\item \emph{$m_a(T)$ from lattice.} 
\LDL{Related  to the previous point, the determination of the temperature dependence 
of the axion mass is a crucial ingredient in order to assess the VRM contribution to axion DM 
abundance. Although in the recent years there have been notable improvements from 
lattice simulations, a final convergence on this problem is desirable and it could 
be realistically achieved in the not so far future.}
%Convergence on $m_a(T)$  behaviour (lattice)
%Reliable  assessment of the existence of a PQ quality problem vs. quantum gravity.
\item \emph{$U(1)_{\rm PQ}$ quality problem.}
%Model building:  

\LDL{Explaining the fundamental origin of the global PQ symmetry and the reason 
why UV physics (in particular quantum gravity) should preserve it at an exceptional good level, 
remains one of the major theoretical issues of the PQ mechanism. 
Although many mechanisms have been proposed so far, 
a convincing way of implementing the PQ symmetry 
as an accidental symmetry in a simple and predictive way 
is still missing. Progress in this direction might reveal unexpected 
connections with quantum gravity or other unsettled issues of the SM.} 

\item \emph{WIMP vs.~axion DM.} \LDL{\bf Bose-Einstein, Sikievie vs.~Davidson... 
However, we should mention also something in the text... }

\item \emph{Stellar cooling anomalies.} 
As we have seen, astrophysical arguments are often very efficient in constraining axion models. 
The future promises to be bright. 
The flourishing of new instrumentation for astrophysical observations promises unprecedented quality in astrophysics data. 
A definite improvement should be expected in the near future from the understanding of the white dwarf population and the construction of reliable WD luminosity functions, which have played an important role in the physics of axions. 
LSST will enlarge considerably the census of WD with respect to GAIA and help in this direction ~\cite{0912.0201}.
The progress with the WD variables is less obvious. 
Though many more variables have been detected~\cite{Corsico:2019nmr}, the secular drift of the oscillation period, $ \dot{P}/P $, has still been measured only for very few of them.
Given the longstanding discrepancy between the measured and expected rate of the period change, which has originated the speculation that another (axion?) cooling mechanism is at play~\cite{Isern:1992gia}, it is certainly desirable to increase the measurements of the secular drift of the oscillation period in many more WD variables.

\item \emph{Supernova.} 
Another longstanding problems that still needs a detailed solution is a reliable understanding of the impact of the observed neutrino signal from SN 1987A on the axion-nucleon coupling. 
This has for a long time been considered the strongest bound on the benchmark axion models. 
Yet, the current results are sill very far from reliable. 
First, there is obviously the problem of the very sparse data.
A new galactic SN explosion would, of course, find us much readier and produce an immensely  more solid data set. 
However, the major problem in this case is with our reduced understanding of the nuclear matter and with a reliable treatment of the reaction rates producing axions from the SN core. 

\end{itemize}
